OmniDrive: A Holistic Vision-Language Dataset for Autonomous Driving with Counterfactual Reasoning

The advances in vision-language models (VLMs) have led to a growing interest in autonomous driving to leverage their strong reasoning capabilities. However, extending these capabilities from 2D to full 3D understanding is crucial for real-world applications. To address this challenge, we propose OmniDrive, a holistic vision-language dataset that aligns agent models with 3D driving tasks through counterfactual reasoning. This approach enhances decision-making by evaluating potential scenarios and their outcomes, similar to human drivers considering alternative actions. Our counterfactual-based synthetic data annotation process generates large-scale, high-quality datasets, providing denser supervision signals that bridge planning trajectories and language-based reasoning. Futher, we explore two advanced OmniDrive-Agent frameworks, namely Omni-L and Omni-Q, to assess the importance of vision-language alignment versus 3D perception, revealing critical insights into designing effective LLM-agents. Significant improvements on the DriveLM Q\&A benchmark and nuScenes open-loop planning demonstrate the effectiveness of our dataset and methods.

==> sec/old1_intro.tex <==
\begin{figure*}[h!]
\vspace{-6mm}
\begin{center}
\includegraphics[scale=0.16]{sec/figures/teaser.pdf}
% \vspace{-5mm}
\caption{
\footnotesize We present OmniDrive, a novel framework for end-to-end autonomous driving with large language model (LLM) agents. Our main contributions involve novel solutions in both model (OmniDrive-Agent) and benchmark (OmniDrive-nuScenes). The former features a novel 3D vision-language model design, whereas the latter is constituted of comprehensive VQA tasks for reasoning and planning.
}%
\label{teaser}
\end{center}
\vspace{-5mm}
\end{figure*}

\section{Introduction}
\label{sec:intro}
The recent rapid development of multimodal LLMs (MLLMs)~\cite{alayrac2022flamingo,li2023blip,liu2023llava} and their excellent reasoning capabilities have led to a stream of applications in end-to-end autonomous driving~\cite{sima2023drivelm,xu2023drivegpt4,wang2023drivemlm,nie2023reason2drive,chen2023driving}. However, the challenge to extend the capabilities from 2D understanding to the intricacies of 3D space is a crucial hurdle to overcome to fully unlock its potential in real-world applications. Understanding and navigating through 3D space is indispensable for autonomous vehicles (AVs) because they directly impact an AV's ability to make informed decisions, anticipate future states, and interact safely with their environment. Although previous works~\cite{marcu2023lingoqa,tian2024drivevlm} have demonstrated successful applications of LLM-agents in autonomous driving, a holistic and principled approach is still needed to fully extend the 2D understanding and reasoning capabilities of MLLMs into complex 3D scenes for understanding the 3D geometry and spatial relations.

Another open issue is the need to address multi-view high resolution video input. On one hand, many current popular 2D MLLM architectures, such as LLaVA-1.5~\cite{liu2023llava,liu2023improvedllava}, can only take $336\times 336$ image input due to the limited vision encoder resolution and LLM token sequence length. Increasing the limitations is not trivial, as it requires significantly more compute and memories. On the other hand, dealing with high resolution video input, oftentimes even multi-view, is a fundamental requirement for long-range AV perception and safe decision making. However, unlike many cloud-based services, real-world industrial autonomous driving applications are mostly on-device and compute-bound. As such, there is a need to design an efficient MLLM architectures with compressed 3D visual representations before feeding to the LLM.

Our answer to the above challenges is a novel Q-Former-styled~\cite{li2023blip} 3D MLLM architecture as shown in ~\cref{teaser}. Unlike LLaVA which adopts a self-attention design, the cross-attention decoder in Q-Former makes it more scalable to higher resolution input by compressing the visual information into sparse queries. Interestingly, we notice that the Q-Former architecture shares considerable similarity with the family of perspective-view models, such as DETR3D~\cite{wang2022detr3d}, PETR(v2)~\cite{liu2022petr,liu2022petrv2}, StreamPETR~\cite{wang2023exploring} and Far3D~\cite{jiang2023far3d}. Using sparse 3D queries, these models have demonstrated considerable advantages over dense bird's-eye view (BEV) representation with leading performance~\cite{wang2023exploring,jiang2023far3d}, long-range perception~\cite{jiang2023far3d} and capability to jointly model map elements~\cite{wu2023topomlp}. The similarity in query-based decoder architecture enables us to align both worlds by appending 3D position encoding to the queries, lifting them to 3D, and attending the multi-view input, as shown in the left portion of Fig.~\ref{teaser}. This process allows the MLLM to gain 3D spatial understanding with minimal efforts and changes, while leveraging the pre-trained knowledge from the abundant images in 2D. 

Besides model architectures, recent drive LLM-agent works also feature the importance of benchmarks~\cite{qian2023nuscenes,marcu2023lingoqa,sima2023drivelm,nie2023reason2drive,ding2024holistic,tian2024drivevlm}. Many of them are presented as question-answering (QA) datasets to train and benchmark the LLM-agent for either reasoning or planning. Despite the various QA setups, benchmarks that involve planning~\cite{sima2023drivelm,ding2024holistic,tian2024drivevlm} still resort to an open-loop setting on real-world sessions (e.g., nuScenes) where expert trajectories are used. Recent studies~\cite{zhai2023rethinking,li2023ego}, however, reveal limitations of open-loop evaluation with implicit biases towards ego status, overly simple planning scenarios, and easy overfit to the expert trajectory. In light of the issue, the proposed benchmark OmniDrive-nuScenes features a counterfactual reasoning benchmark setting where simulated decision and trajectories are leveraged to reason potential consequences. Our benchmark also include other challenging tasks that require full 3D spatial understanding and long-horizon reasoning, as shown in Fig.~\ref{teaser} (right).

In summary, OmniDrive aims to provide a holistic framework for end-to-end autonomous driving with LLM-agents. We propose a principled model design excellent in 3D reasoning and planning, as well as a more challenging benchmark going beyond single expert trajectories.

==> sec/tables/ablation_table_qa.tex <==
\begin{table*}[t!]
\centering
\caption{\textbf{Ablation Study on QA Tasks.} }
\label{ablation_table_qa}
\scalebox{0.8}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multirow{2}{*}{Setting} &
\multicolumn{2}{c|}{Safe} &
\multicolumn{2}{c|}{Red Light} &
\multicolumn{2}{c|}{Collision} &
\multicolumn{2}{c}{Drivable Area}\\
& Precision & Recall & Precision & Recall & Precision & Recall & Precision & Recall \\
\midrule
Full Model& $82.6$ & $24.0$ & $47.7$ & $69.3$ & $27.4$ & $89.8$ & $39.8$& $54.3$\\
\midrule
w/o Attention & $79.6$ & $25.9$ & $45.6$ & $57.7$ & $27.6$ & $90.7$ & $40.0$ & \textbf{$57.8$} \\
\midrule 
w/o Description & \textbf{$84.9$} & $20.0$ & $45.1$ & $75.5$ & $26.9$ & $93.1$ & $39.0$ & $51.0$ \\
\midrule 
w/o Rules & $82.6$ & $23.8$ & \textbf{$49.0$} & $71.1$ & $27.4$ & $92.4$ & $40.6$ & $49.3$ \\
\midrule 
w/o 2D-to-3D & $84.6$ & $19.8$ & $46.1$ & $68.8$ & $26.9$ & \textbf{$94.4$} & $38.6$ & $53.4$ \\
\midrule 
w/o 3D Grounding & $80.4$ & \textbf{$37.0$} & $47.8$ & $68.9$ & $29.0$ & $88.4$ & $40.9$ & $43.7$ \\
\midrule 
w/o Lane-to-Object & $81.4$ & $25.1$ & $44.9$ & $62.6$ & $27.6$ & $92.0$ & $38.4$ & $53.9$ \\
\midrule 
w/o Object-to-Lane & $84.4$ & $25.2$ & $43.5$ & \textbf{$75.1$} & \textbf{$28.3$} & $92.4$ & \textbf{$41.0$} & $54.9$ \\
\bottomrule
\end{tabular}}
\end{table*}

==> sec/tables/algorithm.tex <==


\begin{algorithm}[th!]
\caption{Sampling Trajectories for Counterfactual Reasoning (STCR)}
\begin{algorithmic}[1]
\State \textbf{Input:} Lane centerlines $L_c$, Vehicle intentions $V_i$
\State \textbf{Output:} Final set of sampled trajectories $F_t$

\Procedure{STCR}{}
    \State Construct graph $G$ from $L_c$ using lane-lane topology
    \State $T_l = []$ \Comment{Initialize $T_l$ as an empty list}
    \For{$v \in V_i$}
        \State Select initial lane $l_{init}$ based on $v$
        \State $P \gets$ \Call{DFSPaths}{$G, l_{init}$} \Comment{DFS for all possible paths}
        \For{each $l \in P$}
            \State $B_c \gets$ Interpolate $l$ into a Bezier curve
            \State Initialize $T = []$
            \State $t\_list = $\Call{generate\_t}{completion rates, speed targets}
            \For{each $t$ value in $t\_list$}
                \State Compute position at $t$ using $B_c$ with cubic Bezier formula
                \State $B(t) = (1-t)^3 P_0 + 3(1-t)^2 t P_1 + 3(1-t) t^2 P_2 + t^3 P_3$
                \State $T.append(B(t))$ \Comment{Appending position to trajectory}
            \EndFor
            \State $T_l.append(T)$ \Comment{Appending trajectory $T$ to list $T_l$}
        \EndFor
    \EndFor
    \State Sample trajectories $T_c$ from clustered $T_{all}$
    \State Merge $T_l$ and $T_c$ into list $C_l$
    \State Sample trajectories from $C_l$ to form $F_t$
\EndProcedure

\Function{DFSPaths}{$G, start$}
    \State Initialize paths list $allPaths$
    \State Perform DFS on $G$ from $start$, adding paths to $allPaths$
    \State \Return $allPaths$
\EndFunction

\end{algorithmic}
\label{alg:sample}
\end{algorithm}


==> sec/tables/counter_data.tex <==
\begin{table}[ht]
\centering
\caption{Distribution of Counterfactual Categories in the Validation Set}
\label{counter_analysis}
\scalebox{1.0}{
\setlength{\tabcolsep}{5pt}
\begin{tabular}{l|c|c}
\toprule
\textbf{Counterfactual Category} & \textbf{Count} & \textbf{Percentage (\%)} \\
\midrule
Safe & 9486 & 52.54 \\
\midrule
Out of the drivable area & 4604 & 25.51 \\
\midrule
Collision & 4247 & 23.52 \\
\midrule
Run the red light & 2226 & 12.33 \\
\bottomrule
\end{tabular}}
\end{table}


==> sec/tables/memory.tex <==
\begin{table}
\centering
\caption{Comparison on training memory and time.}
\label{tab:training}
% \tiny
\scalebox{1.0}{
\setlength{\tabcolsep}{5pt}
% \setlength{\tabcolsep}{1.5pt}
\begin{tabular}{c|c|c} 
\toprule
\textbf{Setting} & \textbf{A100 Training Hours} $\downarrow$& \textbf{GPU Memory (G)}$\downarrow$  \\
\midrule
Q-Former3D & \textbf{10} & \textbf{27.0G} \\
Q-Former2D & 13  & 31.7G   \\
\bottomrule
\end{tabular}}
\end{table}
